DIRA: Dynamic Domain Incremental Regularised Adaptation

Autonomous systems (AS) often use Deep Neural Network (DNN) classifiers to allow them to operate in complex, high-dimensional, non-linear, and dynamically changing environments. Due to the complexity of these environments, DNN classifiers may output misclassifications during operation when they face domains not identified during development. Removing a system from operation for retraining becomes impractical as the number of such AS increases. To increase AS reliability and overcome this limitation, DNN classifiers need to have the ability to adapt during operation when faced with different operational domains using a few samples (e.g. 2 to 100 samples). However, retraining DNNs on a few samples is known to cause catastrophic forgetting and poor generalisation. In this paper, we introduce Dynamic Incremental Regularised Adaptation (DIRA), an approach for dynamic operational domain adaption of DNNs using regularisation techniques. We show that DIRA improves on the problem of forgetting and achieves strong gains in performance when retraining using a few samples from the target domain. Our approach shows improvements on different image classification benchmarks aimed at evaluating robustness to distribution shifts (e.g.CIFAR-10C/100C, ImageNet-C), and produces state-of-the-art performance in comparison with other methods from the literature.

==> NN_single_layer_diagramV1.tex <==
\begin{figure}[h!]
    \begin{tikzpicture}[node distance=3.5cm]
 
        % \node (neuron1) [neuron, fill=none, minimum size=2cm, xshift=3.8cm] {$ReLU \Bigg( \mathlarger{\mathlarger{\sum}}_{k=0}^{K} (x_{k,z-1}.w_{x_k,z-1})+b_{k,z})\Bigg)$};
        
        \node (neuron1) [neuron, fill=none, minimum size=2cm, xshift=3.8cm] {$ReLU \Bigg( \mathlarger{\mathlarger{\sum}}_{k=1}^{K} (x_{k}.w_{k})+b\Bigg)$};
        
        %  \node (activation) [process, draw=white, minimum width=4cm, minimum height=2cm, text width=8cm, text height=5cm, text depth = 0 cm, yshift=0cm, xshift=0cm, align=left] {$ReLU(x_{k,z})$};
         
        %  \node (activation) [process, fill=none, minimum width=2cm, minimum height=1cm, yshift=0cm, xshift=7cm, align=center] {{$ReLU(x_{k,z})$}};
    
    
         \draw[arrow] (-0.3,2) -- node[anchor=south, xshift=-0.9cm, yshift =0.3cm] {$x_{1}$} node[anchor=south, yshift =0cm] {$w_{1}$} (1.1,1.3);
         
         \draw[arrow] (-0.3,1) -- node[anchor=south, xshift=-0.9cm, yshift =0.1cm] {$x_{2}$} node[anchor=south, yshift =0cm] {$w_{2}$} (0.9,0.7);
         
         \draw[arrow] (-0.3,0) -- node[anchor=south, xshift=-0.9cm, yshift =-0.3cm] {$x_{3}$} node[anchor=south, yshift =0cm] {$w_{3}$} (0.8,0);
         
         \draw[arrow] (-0.3,-1.5) -- node[anchor=south, xshift=-0.9cm, yshift =-0.6cm] {$x_{K}$} node[anchor=south, yshift =0cm] {$w_{K}$} node[anchor=south,xshift=-0.8cm,yshift =0.5cm] {$.$} node[anchor=south,xshift=-0.8cm,yshift =0.3cm] {$.$} node[anchor=south,xshift=-0.8cm,yshift =0.1cm] {$.$}  (1,-1.1);
         
        % \draw[arrow] (0,1.5) -- node[anchor=south, xshift=-1.3cm, yshift =0.3cm] {$x_{1,}$} node[anchor=south, yshift =0cm] {$w_1$} (2.2,0.6);
         
        %  \draw[arrow] (0,0.75) -- node[anchor=south, xshift=-1.3cm, yshift =0.1cm] {$x_2$} node[anchor=south, yshift =0cm] {$w_2$} (2.1,0.3);
         
        %  \draw[arrow] (0,0) -- node[anchor=south, xshift=-1.3cm, yshift =-0.3cm] {$x_3$} node[anchor=south, yshift =0cm] {$w_3$} (2.05,0); 
        
        %  \draw[arrow] (0,-1.5) -- node[anchor=south, xshift=-1.2cm, yshift =-0.9cm] {$x_K$} node[anchor=south, yshift =0cm] {$w_K$} node[anchor=south,xshift=-1.2cm,yshift =0.3cm] {$.$} node[anchor=south,xshift=-1.2cm,yshift =0.1cm] {$.$} node[anchor=south,xshift=-1.2cm,yshift =-0.1cm] {$.$} %(2.25,-0.6);
        
         
        \draw[arrow] (6.85,0) -- node[anchor=south] {$x_{out}$} (7.5,0);
        
    \end{tikzpicture}
\caption{Artificial neuron in a DNN}
\label{fig:neuron_connected}
\end{figure}


==> RetrainingMethodV1.tex <==
\begin{figure}[h!]
    \begin{tikzpicture}[node distance=3.5cm]
   
    % \node (retraining_method) [process, minimum width=7cm, minimum height=10cm, text width=7cm, text height=10cm, text depth = 0 cm, yshift=0cm, xshift=0cm, align=left] {Retraining method};
    % \node (retraining_method) [process, fill=none, minimum width=4cm, minimum height=5cm, text width=8.4cm, text height=9cm, text depth = 0cm, yshift=-2.4cm, xshift=0cm, align=left] {Retraining method};
    
    \node (training_word) [process, draw=white, minimum width=4cm, minimum height=2cm, text width=8cm, text height=5cm, text depth = 0 cm, yshift=0cm, xshift=0cm, align=left] {Training};
    
    \node (training) [process, fill=none, minimum width=4cm, minimum height=2cm, text width=6cm, text height=0cm, text depth = 3cm, yshift=-1cm, xshift=-1cm, align=left] {\[\mathcal{L}(\theta) = \mathcal{L}_{\text{PoL}}(\theta) + \sum_{j}^{}\dfrac{\lambda_i}{2} F_0(\theta_j - \theta^{*}_{old,j})^2\]\\ \[\theta_{new} = \theta_{old} - \eta_{i} \dfrac{d\mathcal{L}(\theta)}{d\theta}\]};
    
    % \node (shuffle) [process, minimum width=3cm, minimum height=1cm, text width=3cm, text height=0.2cm, text depth = 0cm, yshift=2cm, xshift=2cm] {Shuffle};
    
    \node (change_parameters) [process, minimum width=3cm, minimum height=1.5cm, text width=3cm, text height=0cm, text depth = 0.1cm, yshift=-3.7cm, xshift=0.5cm] {Change tuning parameters ($\lambda_i$, $\eta_i$)};
    
    \node (criteria_assessment) [process, minimum width=8cm, minimum height=1.5cm, text width=8cm, text height=0.2cm, text depth = 0 cm, yshift=-6cm, xshift=0cm] {Criteria assessment};
    
    \draw[arrow] (-3,1.5) -- node[anchor=east,yshift=0.2cm] {$M_0$} (-3,0.6);
    
    \draw[arrow] (-3,-2.61) -- node[anchor=east] {$M_i$} (-3,-5.25);
    
    \draw[arrow] (0.5,-5.25) -- node[anchor=east,xshift=1.3cm,yshift =-0.6cm] {(if not satisfied)} (0.5,-4.45);
    \draw[arrow] (0.5,-2.95) -- node[anchor=east] {} (0.5,-2.61);
    
    % \draw[arrow] (2,3.5) -- node[anchor=east] {$[S_1,...,S_{i}]$} (2,2.5);
    
    % \draw[arrow] (0.9,1.5) -- node[anchor=east] {$[S_{(1,...,i),train}]$} (0.9,0.6);
    %  \draw[arrow] (3.1,1.5) -- node[anchor=east, yshift=2.92cm] {$[S_{(1,...,i),test}]$} (3.1,-5.25);
    
      \draw[arrow] (0.7,1.5) -- node[anchor=east, yshift=0.2cm] {$[S_{\text{PoL, }train}]$} (0.7,0.6);
      
     \draw[arrow] (2.4,1.5) -- node[anchor=east, yshift=3.1cm] {$[S_{\text{PoL, }test}]$} (2.4,-5.25);
    
     \draw[arrow] (3.8,1.5) -- node[anchor=east, yshift=3.1cm] {$[S_{0,test}]$} (3.8,-5.25);
     
     \draw[arrow] (0,-6.75) -- node[anchor=east,yshift =-0.5cm] {$M_i$} (0,-8);
     \draw[arrow] (0,-6.75) -- node[anchor=east,xshift=1cm,yshift =0.8cm] {(if satisfied)} (0,-8);
    
    
    % \node (training) [process, fill=none, minimum width=4cm, minimum height=5cm, text width=6cm, text height=0cm, text depth = 2cm, yshift=0cm, xshift=0cm, align=left] {\[\mathcal{L}(\theta) = \mathcal{L}_{new}(\theta) + \sum_{j}^{}\dfrac{\lambda_i}{2} F_0(\theta_j - \theta^{*}_{old,j})^2\]\\ \[\theta_{new} = \theta_{old} - lr_{i} \dfrac{d\mathcal{L}(\theta)}{d\theta}\]};
    
    % \node (assessment_criteria) [process, minimum width=1.5cm, minimum height=5cm, text width=1.7cm, text height=0cm, text depth = 0 cm, yshift=0cm, xshift=2.5cm] {Assessment criteria};
    % draw=black
    % \draw [arrow] (-4.5,0) --  node[anchor=south] {$[S_{0,test}]$} (-4,0);
    
    % \node (original_dataset_train) [process, minimum width=1.25cm, text width=1.3cm, yshift=-0.25cm, xshift=-0.9cm] {[$S_{0,train}$]};
    
    % \mathcal{L}(\theta) = \mathcal{L}_{B}(\theta) +  \sum_{i}^{} \frac{\lambda}{2} F^A_i (\theta_i - \theta^{*}_{A,i})^2
    
    % \draw [arrow] (initial_training) -- (initial_model);
    
    % \draw[arrow] (-0.75,-3.75) -- node[anchor=east] {$i=0$} (-0.75,-5.65);
    % \[ \sum_{n=1}^{\infty} 2^{-n} = 1 \]
    % \[\sum_{t=0}^{n}\dfrac{CF_t}{(1+r)^t}\]
    % $\mathcal{L}(\theta) = \mathcal{L}_{new}(\theta) + \sum{j}{}\lambda_i F_0(\theta_j - \theta^{*}_{old,j})^2$
    
    \node (retraining_method) [process, fill=none, minimum width=4cm, minimum height=5cm, text width=8.4cm, text height=8.0cm, text depth = 0cm, yshift=-3.2cm, xshift=0cm, align=left] {Retraining method};
    \end{tikzpicture}
\caption{Retraining Method}
\label{fig:retraining_method2}
\end{figure}


==> RetrainingPipelineV1.tex <==
\begin{figure}[h!]
    \begin{tikzpicture}[node distance=3.5cm]
   
    \node (original_dataset) [process, minimum width=3.5cm, minimum height=1.75cm, text width=3.3cm, text height=0cm, text depth = 1 cm, yshift=0cm, xshift=0cm, align=left] {Original dataset [$S_0$]};
    
    \node (original_dataset_train) [process, minimum width=1.25cm, text width=1.3cm, yshift=-0.25cm, xshift=-0.9cm] {[$S_{0,train}$]};
    
    \node (original_dataset_test) [process,  minimum width=1.25cm, text width=1.3cm, yshift=-0.25cm, xshift=0.9cm] {[$S_{0,test}$]};
    
    \node (initial_training) [process,  below of=original_dataset , yshift=1.75cm, xshift=0cm] {Initial training};
    
    \node (initial_model) [process,  below of=initial_training , yshift=2cm, xshift=0cm] {Initial model $(M_0)$};
    
    \node (retraining_method) [process, minimum width=7cm,  below of=initial_model , yshift=2cm, xshift=3.3cm] {Retraining method};
    
    \node (latest_model) [process, minimum width=8.6cm,  below of=initial_model , yshift=0.6cm, xshift=2.5cm] {Latest model $(M_{i})$};
    
    \node (new_instance) [process,  right of=initial_training, text width=3.3cm, yshift=2.15cm, xshift=1.5cm] {New instance [$S_{i}$]};
    
    % \node (oversampling) [process,  below of=new_instance, text width=3.3cm , yshift=2cm, xshift=0cm] {Create a distribution (Oversampling)};
    
    \node (PoL_tasks) [process, minimum width=3.5cm, minimum height=1.5cm, text width=3.5cm, text height=0cm, text depth = 0.9 cm, yshift=-1.45cm, xshift=5cm, align=left] {PoL tasks};
    
    \node (new_instances_storage) [process,  below of=new_instance, text width=3.3cm , yshift=1.5cm, xshift=0cm] {Accumulated new instances $[S_1,...,S_{i}]$};
    
    \node (shuffle) [process, minimum width=3cm, minimum height=1cm, text width=3cm, text height=0.2cm, text depth = 0cm, yshift=-3.0cm, xshift=5cm] {Shuffle};
    
      \draw[arrow] (4.1,-3.5) -- node[anchor=east] {$[S_{\text{PoL, }train}]$} (4.1,-4.25);
      
     \draw[arrow] (6.1, -3.5) -- node[anchor=east, yshift=0cm] {$[S_{\text{PoL, }test}]$} (6.1,-4.25);
    
    \draw [arrow] (original_dataset) -- (initial_training);
    
    \draw [arrow] (initial_training) -- (initial_model);
    
    \draw[arrow] (-0.75,-3.75) -- node[anchor=east] {$i=0$} (-0.75,-5.65);
    
    \draw[arrow] (0.75,-3.75) -- (0.75,-4.25);
    
    \draw[arrow] (3.3,-5.25) -- node[anchor=east] {$i>0$} (3.3,-5.65);
    
    % \draw [arrow] (original_dataset_test) -| node[anchor=south] {$S_{0,test}$} (2.5,-4.25);
    
    \draw [arrow] (original_dataset_test) -| (2.1,-4.25);
    
    \draw [arrow] (new_instance) -- (new_instances_storage);
    
    % \draw [arrow] (oversampling) -- (new_instances_storage);
    
    \draw [arrow] (new_instances_storage) -- (5,-2.5);

    \end{tikzpicture}
\caption{Retraining Pipeline}
\label{fig:retraining_pipeline2}
\end{figure}


==> RetrainingSetsGenerationV1.tex <==
\begin{figure*}[h!]
    \begin{tikzpicture}[node distance=3.5cm]
   
    \node (mnist_dataset) [process, minimum width=3.5cm, minimum height=1.4cm, text width=3.3cm, text height=0cm, text depth = 0.7cm, yshift=0cm, xshift=0cm, align=left] {MNIST dataset};
    
    \node (new_tasks_train) [process, minimum width=1.25cm, minimum height=0.7cm, text width=1.3cm, yshift=-0.2cm, xshift=-0.9cm] {[$S_{0,train}$]};
    
    \node (new_tasks_test) [process, minimum width=1.25cm, minimum height=0.7cm, text width=1.3cm, yshift=-0.2cm, xshift=0.9cm] {[$S_{0,test}$]};
    
    % \node (original_dataset) [process, minimum width=3.5cm, minimum height=1.75cm, text width=2.3cm, text height=0cm, text depth = 0 cm, yshift=0cm, xshift=5cm, align=left] {Original dataset};
    
    % \node (new_tasks_train) [process, minimum width=1.25cm, minimum height=0.7cm, text width=1.3cm, yshift=-0.5cm, xshift=9cm] {[$S_{0,train}$]};
    
    % \node (new_tasks_test) [process, minimum width=1.25cm, minimum height=0.7cm, text width=1.3cm, yshift=0.5cm, xshift=9cm] {[$S_{0,test}$]};
    
    \node (nmnist_dataset) [process, minimum width=3.5cm, minimum height=4cm, text width=3.3cm, text height=0cm, text depth = 3.3cm, yshift=-3.2cm, xshift=0cm, align=left] {N-MNIST dataset};
    
    \node (noisy1) [process, minimum width=3cm, minimum height=0.7cm, text width=3cm, yshift=-2.2cm, xshift=0cm] {Noisy dataset 1 (Gaussian noise)};
    
     \node (noisy2) [process, minimum width=3cm, minimum height=0.7cm, text width=3cm, yshift=-3.4cm, xshift=0cm] {Noisy dataset 2  (Blur noise)};
     
     \node (noisy3) [process, minimum width=3cm, minimum height=0.7cm, text width=3cm, yshift=-4.6cm, xshift=0cm] {Noisy dataset 3 (Contrast noise)};
    
    % \node (noisy2) [process, minimum width=3cm, minimum height=0.7cm, text width=3cm, yshift=-3.4cm, xshift=0cm] {Noisy dataset 1 (Blur noise)};
    
    % \node (new_tasks_test) [process, minimum width=1.25cm, minimum height=0.7cm, text width=1.3cm, yshift=-4cm, xshift=0.9cm] {[$S_{0,test}$]};
    
     \node (retraining_sets_generator) [process, minimum width=12cm, minimum height=4cm, text width=12cm, text height=3.7cm, text depth = 0cm, yshift=-3.2cm, xshift=9cm, align=left] {Retraining sets generator};

%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \node (random_instances) [process, minimum width=3cm, minimum height=3.3cm, text height=3cm, text depth = 0cm, yshift=-3cm, xshift=4.5cm, align=left] {Random instances};
    
     \node (i_1) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2cm, xshift=3.7cm] {};
     
     \node (i_2) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2.3cm, xshift=4cm] {};
     
     \node (i_3) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2.6cm, xshift=4.3cm] {};
     
     \node (i_4) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2.9cm, xshift=4.6cm] {};
     
     \node (i_5) [process, minimum width=1cm, minimum height=0.8cm, yshift=-3.1cm, xshift=4.9cm] {};
     
     \node (i_6) [process, minimum width=1cm, minimum height=0.8cm, yshift=-3.4cm, xshift=5.2cm] {};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%     
     \node (oversampling) [process, minimum width=8cm, minimum height=3.3cm, text width = 8cm, text height=3cm, text depth = 0cm, yshift=-3cm, xshift=10.8cm, align=left] {Oversampling (small rotation + shift)};
    
     \node (ii_1) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2cm, xshift=8.2cm] {};
     
     \node (ii_2) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2.3cm, xshift=8.5cm] {};
     
     \node (ii_3) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2.6cm, xshift=8.8cm] {};
     
     \node (ii_4) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2.9cm, xshift=9.1cm] {};
     
     \node (ii_5) [process, minimum width=1cm, minimum height=0.8cm, yshift=-3.1cm, xshift=9.4cm] {};
     
     \node (ii_6) [process, minimum width=1cm, minimum height=0.8cm, yshift=-3.4cm, xshift=9.7cm] {};
     
     \node[label={[label distance=0.5cm,text depth=-1ex,rotate=0]right:. . .}] at (10,-2.7) {};
     
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \node (iii_1) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2cm, xshift=12.2cm] {};
     
     \node (iii_2) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2.3cm, xshift=12.5cm] {};
     
     \node (iii_3) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2.6cm, xshift=12.8cm] {};
     
     \node (iii_4) [process, minimum width=1cm, minimum height=0.8cm, yshift=-2.9cm, xshift=13.1cm] {};
     
     \node (iii_5) [process, minimum width=1cm, minimum height=0.8cm, yshift=-3.1cm, xshift=13.4cm] {};
     
     \node (iii_6) [process, minimum width=1cm, minimum height=0.8cm, yshift=-3.4cm, xshift=13.7cm] {};
     
    %  \node (i_7) [process, minimum width=1cm, minimum height=0.8cm, yshift=-4.0cm, xshift=5.8cm] {};
     
    %  \node (noisy3) [process, minimum width=3cm, minimum height=0.7cm, text width=3cm, yshift=-4.6cm, xshift=0cm] {Noisy dataset 3 (Contrast noise)};
   
    
    \draw[arrow] (7.5,-4) -- node[anchor=east] {} (7.5,-1.5);
    \node[label={[label distance=0.5cm,text depth=-1ex,rotate=90]right:Oversamples}] at (7,-4.2) {};
    
    \draw[arrow] (7.5,-4) -- node[anchor=north] {} (14,-4);
    \node[label={[label distance=0.5cm,text depth=-1ex,rotate=0]right:New instance}] at (12,-4.2) {};
  
    \node (retraining_sets) [process, minimum width=1.5cm, minimum height=0.7cm, text width=1.5cm, yshift=-3.2cm, xshift=15.15cm] {Retraining sets};
    
    \end{tikzpicture}
\caption{Retraining sets generation}
\label{fig:retraining_sets}
\end{figure*}


==> other/figures/retraining_framework.tex <==
\begin{figure*}[]
    \begin{tikzpicture}[node distance=3.5cm]
     
    \node (augmentation) [process, fill=none, minimum width=2cm, minimum height=1.5cm, text width=2cm, text height=0cm, text depth = 0.1cm, yshift=0cm, xshift=0cm, align=center] {Data \\Augmentation};

    \node (training) [process, fill=none, right of=augmentation, minimum width=4cm, minimum height=2cm, text width=6cm, text height=0cm, text depth = 3cm, yshift=-2cm, xshift=2cm, align=left] {\[\mathcal{L}(\theta) = \mathcal{L}_{\text{PoL}}(\theta) + \sum_{j}^{}\dfrac{\lambda_i}{2} F_0(\theta_j - \theta^{*}_{old,j})^2\]\\ \[\theta_{new} = \theta_{old} - \eta_{i} \dfrac{d\mathcal{L}(\theta)}{d\theta}\]};

    \node (training_word) [process, , draw=none, fill=none, right of=augmentation, minimum width=0cm, minimum height=0cm, text width=6cm, text height=0cm, text depth = 0cm, yshift=-3.5cm, xshift=2cm, align=left] {Training};


    \node (CAS) [process, fill=none, right of=augmentation, minimum width=2cm, minimum height=1.5cm, text width=2cm, text height=0cm, text depth = 0.1cm, yshift=0cm, xshift=8cm, align=center] {CAS \\Assessment};

    \node (change_parameters) [process, fill=none, below of =CAS, minimum width=2cm, minimum height=2cm, text width=2cm, text height=0cm, text depth = 0.95cm, yshift=1cm, xshift=0cm, align=center] {Change tuning parameters ($\lambda_i$, $\eta_i$)};
    

    \draw[arrow] (-2,0) -- node[anchor=west,xshift=-0.3cm,yshift=0.2cm] {$N_T$} (augmentation);

    \draw[arrow] (1.1,0.5) -- node[anchor=west,xshift=-4.7cm,yshift=0.2cm] {$S_{T,test}$} (10.4,0.5);

    \draw[arrow] (1.1,-0.6) -- node[anchor=west,xshift=-0.7cm,yshift=0.2cm] {$S_{T,train}$} (2.4,-0.6);

    \draw[arrow] (8.6,-0.6) -- node[anchor=west,xshift=-0.5cm,yshift=0.2cm] {$M_{I}$} (10.4,-0.6);

    \draw[arrow] (CAS) -- node[anchor=west,xshift=0cm,yshift=0cm] {$CAS<K$} (change_parameters);

    \draw[arrow] (CAS) -- node[anchor=west,xshift=-1.2cm,yshift=0.2cm] {$CAS>K$} (15,0);

    \draw[arrow] (CAS) -- node[anchor=west,xshift=1.2cm,yshift=0cm] {$M_T$} (15,0); 

    \draw[arrow] (change_parameters) -- node[anchor=west,xshift=1.2cm,yshift=0cm] {} (8.6,-2.5); 

    \draw[arrow] (-2,-1.5) -- node[anchor=west,xshift=-2cm,yshift=0.2cm] {$M_0$} (2.4,-1.5); 

    \draw[arrow] (-2,-2.5) -- node[anchor=west,xshift=-2cm,yshift=0.2cm] {$X_{0,test}$} (2.4,-2.5); 


    \end{tikzpicture}
\caption{DIRA Retraining Framework}
\label{fig:retraining_method2}
\end{figure*}

